90 GHz Continuum Observations of Messier 66

Radio emission at around 90 GHz from star-forming galaxies is expected to be strongly dominated by the free-free component due to ionising radiation from massive, short-lived, stars. We present high surface-brightness sensitivity observations at 90 GHz of the nearby star-forming galaxy Messier 66 with resolution of about 9 arcsec (corresponding to a physical scale of about 500 pc) and analyse these observations in combination with archival lower frequency radio and mid-infrared measurements. For the four regions for which the observations support our models we find that the free-free component indeed dominates the emission at 90 GHz, making up 76--90 per cent of the luminosity at this frequency but with the data also consistent with all of the emission being due to free-free. The estimates of free-free luminosities are also consistent, within measurement and decomposition errors, with star-formation rates derived from lower radio frequencies and mid-infrared observations. In our analysis we consider both power-law and curved spectra for the synchrotron component but do not find evidence to support the curved model in preference to the power-law.

==> versioninfo.tex <==
\newcommand{\bzrrevid}{bojan@bnikolic.co.uk-20120508182116-4f71t2vhxjudzxz6}
\newcommand{\bzrdate}{2012-05-08 19:21:16 +0100}
\newcommand{\bzrrevno}{125}
\newcommand{\bzrbranchnick}{2011-M66-letter}

